How Much Can CLIP Benefit Vision-and-Language Tasks?

Most existing Vision-and-Language (V&L) models rely on pre-trained visual encoders, using a relatively small set of manually-annotated data (as compared to web-crawled data), to perceive the visual world. However, it has been observed that large-scale pretraining usually can result in better generalization performance, e.g., CLIP (Contrastive Language-Image Pre-training), trained on a massive amount of image-caption pairs, has shown a strong zero-shot capability on various vision tasks. To further study the advantage brought by CLIP, we propose to use CLIP as the visual encoder in various V&L models in two typical scenarios: 1) plugging CLIP into task-specific fine-tuning; 2) combining CLIP with V&L pre-training and transferring to downstream tasks. We show that CLIP significantly outperforms widely-used visual encoders trained with in-domain annotated data, such as BottomUp-TopDown. We achieve competitive or better results on diverse V&L tasks, while establishing new state-of-the-art results on Visual Question Answering, Visual Entailment, and V&L Navigation tasks. We release our code at https://github.com/clip-vil/CLIP-ViL.

==> algo.tex <==
\begin{algorithm}[t]
\DontPrintSemicolon
\caption{Hessian AWare Quantization}
\label{alg:hq}
    \SetAlgoLined
    \KwInput{Block-wise Hessian eigenvalues $\lambda_i$ (computed from~\aref{alg:power_iteration}), and block size $n_i$ 
    for $i=1,\cdots,b$.

    }

    \For(\tcp*[h]{Compute Quantization Precision}){i $=1,2,\ldots, b$}{

        $S_i = \lambda_i/n_i$ \tcp*{See~\eref{eqn:define_S}}
    }
    
    
    Order $S_i$ in descending order and to determine relative quantization precision for each block.
    
    Compute $\Delta W_i$ based on~\eref{eqn:quantization_function}.

    \For(\quad \quad \quad\quad\quad \tcp*[h]{Fine-Tuning Order}){i $=1,2,\ldots, b$}{
       $\Omega_i = \lambda_i\|\Delta W_i\|^2$ \tcp*{See~\eref{eqn:define_O}}
    }
    
    Order $\Omega_i$ in descending order and perform block-wise fine-tuning
\end{algorithm}




